From Fixed Keys to Readable Schemas: Small Language Models for Vehicle Agent Function Calls

In-vehicle assistants must translate natural-language requests into accurate vehicle function calls under strict memory and latency constraints, making small language models (SLMs) attractive for on-device deployment. For such models, a key design choice is how the available function surface is presented. Two approaches are to represent each function with a dedicated Functional Token (FT) or provide function schemas directly in the prompt. FTs enable compact inference but are restricted to functions learned during training, whereas Schema-in-Prompt (SIP) can generalize to unseen functions at the cost of longer prompts and higher inference overhead. We introduce a benchmark of 9,822 single-turn examples spanning 79 vehicle functions derived from Android Automotive, including held-out functions and requests requiring refusal. We compare both approaches under matched fine-tuning across four SLMs from 270M to 1.7B parameters. On functions seen during training, scaling provides limited benefit: the 270M model can match the 1.7B model, and the highest Seen accuracy in our main grid occurs at 0.6B. On held-out functions, FT achieves zero accuracy by construction, whereas SIP generalizes and improves substantially with scale. On out-of-scope requests, FT can invoke an unavailable function it was trained to emit, while SIP more reliably refuses based on the functions offered. This flexibility comes with a higher inference cost, chiefly the latency of processing the schema prompt. Our theoretical analysis formalizes why only SIP can predict functions withheld as training targets and why longer schema contexts increase inference cost. Overall, function-surface representation, rather than model scale alone, determines the capabilities and failure modes of SLM-based vehicle function calling.

==> tables/corpusmacros.tex <==
% Generated by vfc.eval.corpus. Do not edit; re-run `make corpus`.
% \vfccorpus{examples} -> the corpus size; see vfc/eval/corpus.py for the keys.
\makeatletter
\providecommand{\vfc@missing}[2]{\textbf{??#1/#2??}}
\newcommand{\vfccorpus}[1]{%
  \ifcsname vfccorpus@#1\endcsname\csname vfccorpus@#1\endcsname\else\vfc@missing{corpus}{#1}\fi}
\expandafter\gdef\csname vfccorpus@distinctutterances\endcsname{yes}
\expandafter\gdef\csname vfccorpus@eval\endcsname{3{,}225}
\expandafter\gdef\csname vfccorpus@examples\endcsname{9{,}822}
\expandafter\gdef\csname vfccorpus@functions\endcsname{79}
\expandafter\gdef\csname vfccorpus@notoffered\endcsname{999}
\expandafter\gdef\csname vfccorpus@offeredmax\endcsname{24}
\expandafter\gdef\csname vfccorpus@offeredmedian\endcsname{14}
\expandafter\gdef\csname vfccorpus@offeredmin\endcsname{4}
\expandafter\gdef\csname vfccorpus@outofscope\endcsname{2{,}155}
\expandafter\gdef\csname vfccorpus@outofscopeeval\endcsname{533}
\expandafter\gdef\csname vfccorpus@outofscopefunctions\endcsname{5}
\expandafter\gdef\csname vfccorpus@outofscopenamed\endcsname{65}
\expandafter\gdef\csname vfccorpus@outofscopetargetfunctions\endcsname{--}
\expandafter\gdef\csname vfccorpus@outofscopetrain\endcsname{1{,}622}
\expandafter\gdef\csname vfccorpus@seen\endcsname{5{,}521}
\expandafter\gdef\csname vfccorpus@seeneval\endcsname{546}
\expandafter\gdef\csname vfccorpus@seenfunctions\endcsname{56}
\expandafter\gdef\csname vfccorpus@seentargetfunctions\endcsname{56}
\expandafter\gdef\csname vfccorpus@seentrain\endcsname{4{,}975}
\expandafter\gdef\csname vfccorpus@sliceafterrepair\endcsname{15}
\expandafter\gdef\csname vfccorpus@sliceblind\endcsname{202}
\expandafter\gdef\csname vfccorpus@slicefaithful\endcsname{217}
\expandafter\gdef\csname vfccorpus@slicefaithfulrate\endcsname{100.0\%}
\expandafter\gdef\csname vfccorpus@slicerepaired\endcsname{9}
\expandafter\gdef\csname vfccorpus@slicereviewed\endcsname{217}
\expandafter\gdef\csname vfccorpus@slicestrata\endcsname{42}
\expandafter\gdef\csname vfccorpus@sliceunambiguous\endcsname{215}
\expandafter\gdef\csname vfccorpus@sliceunambiguousrate\endcsname{99.1\%}
\expandafter\gdef\csname vfccorpus@surfaceversion\endcsname{0.3.2}
\expandafter\gdef\csname vfccorpus@targetfunctions\endcsname{74}
\expandafter\gdef\csname vfccorpus@train\endcsname{6{,}597}
\expandafter\gdef\csname vfccorpus@unseen\endcsname{2{,}146}
\expandafter\gdef\csname vfccorpus@unseeneval\endcsname{2{,}146}
\expandafter\gdef\csname vfccorpus@unseenfunctions\endcsname{18}
\expandafter\gdef\csname vfccorpus@unseentargetfunctions\endcsname{18}
\expandafter\gdef\csname vfccorpus@unseentrain\endcsname{0}
\expandafter\gdef\csname vfccorpus@vehiclecannot\endcsname{1{,}156}
\makeatother


==> tables/pvalues.tex <==
% Generated by vfc.eval.significance. Do not edit; re-run `make significance`.
% Cite one in prose as \vfcp{parity-270m-vs-17b}{0}. A missing key renders a loud ??.
\makeatletter
\providecommand{\vfc@missing}[2]{\textbf{??#1/#2??}}
\newcommand{\vfcp}[2]{%
  \ifcsname vfcp@#1@#2\endcsname\csname vfcp@#1@#2\endcsname\else\vfc@missing{#1}{#2}\fi}

\expandafter\gdef\csname vfcp@parity-270m-vs-17b@0\endcsname{0.607}
\expandafter\gdef\csname vfcp@parity-270m-vs-17b@1\endcsname{0.267}
\expandafter\gdef\csname vfcp@parity-270m-vs-17b@2\endcsname{0.238}
\expandafter\gdef\csname vfcp@parity-270m-vs-06b@0\endcsname{0.180}
\expandafter\gdef\csname vfcp@parity-270m-vs-06b@1\endcsname{0.065}
\expandafter\gdef\csname vfcp@parity-270m-vs-06b@2\endcsname{0.013}
\expandafter\gdef\csname vfcp@specialised-seen@0\endcsname{0.453}
\expandafter\gdef\csname vfcp@specialised-seen@1\endcsname{1.000}
\expandafter\gdef\csname vfcp@specialised-seen@2\endcsname{0.581}
\expandafter\gdef\csname vfcp@specialised-unseen@0\endcsname{4.5 \times 10^{-4}}
\expandafter\gdef\csname vfcp@specialised-unseen@1\endcsname{5.6 \times 10^{-6}}
\expandafter\gdef\csname vfcp@specialised-unseen@2\endcsname{4.8 \times 10^{-6}}
\expandafter\gdef\csname vfcp@native-format-unseen@0\endcsname{3.6 \times 10^{-5}}
\expandafter\gdef\csname vfcp@native-format-unseen@1\endcsname{3.9 \times 10^{-12}}
\expandafter\gdef\csname vfcp@native-format-unseen@2\endcsname{5.8 \times 10^{-23}}
\expandafter\gdef\csname vfcp@lora-vs-fullft-unseen@0\endcsname{2.3 \times 10^{-46}}
\expandafter\gdef\csname vfcp@lora-vs-fullft-unseen@1\endcsname{4.3 \times 10^{-66}}
\expandafter\gdef\csname vfcp@lora-vs-fullft-unseen@2\endcsname{0.084}

% The weakest seed of a comparison, for prose that says "all three seeds, worst p".
% Generated rather than picked by hand: which seed is weakest can change on a re-run,
% and a sentence naming one by number would go quietly wrong.
\newcommand{\vfcpmax}[1]{%
  \ifcsname vfcpmax@#1\endcsname\csname vfcpmax@#1\endcsname\else\vfc@missing{#1}{max}\fi}
\expandafter\gdef\csname vfcpmax@lora-vs-fullft-unseen\endcsname{0.084}
\expandafter\gdef\csname vfcpmax@native-format-unseen\endcsname{3.6 \times 10^{-5}}
\expandafter\gdef\csname vfcpmax@parity-270m-vs-06b\endcsname{0.180}
\expandafter\gdef\csname vfcpmax@parity-270m-vs-17b\endcsname{0.607}
\expandafter\gdef\csname vfcpmax@specialised-seen\endcsname{1.000}
\expandafter\gdef\csname vfcpmax@specialised-unseen\endcsname{4.5 \times 10^{-4}}
\makeatother

